ProtAlign: Contrastive learning paradigm for Sequence and structure alignment

Protein language models often take into consideration the alignment between a protein sequence and its textual description. However, they do not take structural information into consideration. Traditional methods treat sequence and structure separately, limiting the ability to exploit the alignment between the structure and protein sequence embeddings. In this paper, we introduce a sequence structure contrastive alignment framework, which learns a shared embedding space where proteins are represented consistently across modalities. By training on large-scale pairs of sequences and experimentally resolved or predicted structures, the model maximizes agreement between matched sequence structure pairs while pushing apart unrelated pairs. This alignment enables cross-modal retrieval (e.g., finding structural neighbors given a sequence), improves downstream prediction tasks such as function annotation and stability estimation, and provides interpretable links between sequence variation and structural organization. Our results demonstrate that contrastive learning can serve as a powerful bridge between protein sequences and structures, offering a unified representation for understanding and engineering proteins.

==> sections/intro.tex <==

\begin{figure*}
    \centering
    \begin{tabular}{cc}
           \adjincludegraphics[width=0.47\textwidth, trim={6cm 7cm 10cm 5cm}, clip]{Figures/model-diagram 1.pdf} &\hspace{-10mm}\adjincludegraphics[width=0.47\textwidth, trim={11cm 6cm 3cm 4cm}, clip]{Figures/icassp-diagram-framework_v2.pdf} \\
           (a) Sequence/Structure model. & (b) Contrastive learning.
    \end{tabular}

    \caption{{\bf ProtAlign}. Fig. (a) shows our proposed model consisting of multi-head self-attention (MSA) layer and LayerNorm layer, with the learnable token as queries, structure/sequence embeddings as keys and values within the MSA layer. Fig. (b) shows the alignment protocol for training our model.}
    \label{fig:framework}
\end{figure*}

\added{Understanding the relationship between a protein’s sequence and its three-dimensional structure is a central problem in computational biology~\cite{seqstructrelation}. Over the past few years, advances in machine learning and deep learning have driven striking improvements in predicting and reasoning about protein structures from sequence information~\cite{af3}. While these advances have largely focused on predicting structures from sequences, more recent efforts extend the scope of protein representation learning. A prominent direction is to pair protein sequences with textual modalities, where natural language annotations provide functional or contextual information that complements sequence data~\cite{}. Consequently, these multi-modal \texttt{protein language models} have opened new avenues to better understand the sequence and Approaches such as EvoLlama~\cite{evollama} incorporate the protein sequence and structural information through their respective encoders into the textual domain.}

More recently, models such as EvoLlama \cite{evollama} try to incorporate protein the sequence and structural information in a textual context setting using Llama \cite{llama}. They feed a pre-trained Protein-MPNN \cite{proteinmpnn} encoder with the sequence information, and a pretrained ESM2 \cite{esm2} encoder, calculate the mean across the sequences, project the embeddings to a common dimensionality and concatenate the two embeddings, which is then fed it to an LLM like Llama\cite{llama} for inference. However, given these two embeddings represent two very different modalities, there might not be any alignment between them causing the LLM to misunderstand the relation between the protein sequence and its structure.

In another work, Boado et al.\ \cite{concat-alignment} use the sequence and structure as inputs to an EGNN model, which predicts the GO (Gene Ontology) functions. However, there is no alignment done between the sequence and structure embeddings and are naively fed to the EGNN. 

Several studies have explored the alignment of protein sequences with their textual descriptions through a contrastive learning paradigm [see \cite{protst, protclip}]. However, there are few that consider the alignment between a sequence and structure. Reference \cite{Teng2024} aims to align more than two modalities- 2D graphs, text description, 3D protein pocket, 3D molecular conformation through contrastive loss-guided training. Later, these aligned embeddings are utilized for zero-shot prediction tasks such as cross-modal retrieval.

 Boado et al.\ \cite{alignment} were the first to consider the alignment between a protein sequence and its corresponding structure. In this work, the authors pre-trained an Multi-Layer Perceptron to align a protein structure and sequence, among many other features such as protein functions, with the ultimate downstream task of predicting gene ontology. However, there was no evidence of results or how this pre-training was performed. 


Thus we define our \textbf{problem statement} - How can protein sequences and its structures be aligned over a common embedding space in a multi-modal setting. We list the contributions of this paper below.

\begin{itemize}
    \item We develop a novel alignment model using a multi-head attention model for projecting into a common embedding space. 
    \item We develop a contrastive loss style training around our proposed model architecture for aligning the protein sequence embeddings and its corresponding structures. 
    \item We present interpretable results, which, using dimensionality reduction techniques, show the improvement in proximity of the embeddings from different modalities. 
\end{itemize}
To tackle all of the above contributions, we introduce \textbf{ProtAlign}, a novel sequence-structure approach that aligns a protein seqeuence with its corresponding structure, but exploiting the attention features across the sequence and structure.

% \noindent \textbf{Related Work.}

% Traditional methods like \cite{Amy2020} focuses on leveraging information inherent in the sequence modality only for downstream tasks. Recent works \cite{protst, protclip} focuses on aligning protein sequences and textual descriptions to learn a unified representation, which can be better utilized in downstream applications.
% Reference \cite{concat-alignment}  leverages both sequence and structure information to predict Gene Ontology (GO) function. However, they simply combine the features from these two modalities, without aligning them in a unified embedding space.


==> sections/related.tex <==
\textcolor{red}{There has been some very recent work \cite{alignment} where Boado et al.\ consider the alignment between a protein sequence and its corresponding structure. In this work, the authors pre-train the models to be aligned with protein structure and sequence, among many other features such as gene ontology and protein functions. However, they do not report their pretrained statistics and do not elaborate on how this structure sequence alignment is done. This makes it hard for us to compare against this approach.}


{\color{blue} Hasin: Added some relevant works here. 

Traditional methods like \cite{Amy2020} focuses on leveraging information inherent in the sequence modality only for downstream tasks. Recent works \cite{protst, protclip} focuses on aligning protein sequences and textual descriptions to learn a unified representation, which can be better utilized in downstream applications.
Reference \cite{concat-alignment}  leverages both sequence and structure information to predict Gene Ontology (GO) function. However, they simply combine the features from these two modalities, without aligning them in a unified embedding space.
Reference \cite{Teng2024} aims to align more than two modalities- 2D graphs, text description, 3D protein pocket, 3D molecular conformation through contrastive loss-guided training. Later, these aligned embeddings are utilized for zero-shot prediction tasks such as cross-modal retrieval.
}
  
% A significant amount of work has been done in the field of aligning protein sequences with their structures. For example, Boado et al.\ \cite{Boadu2023} `TransFun', a transformer-based protein language model to learn ontology functions of protein structures. Similarly, Zhou et al.\ \cite{Xu2023} train a cross-attention model to align protein sequence against their \cite{Zhou2025, Xue2021}



